VoicePAT: An Efficient Open-source Evaluation Toolkit for Voice Privacy Research

Speaker anonymization is the task of modifying a speech recording such that the original speaker cannot be identified anymore. Since the first Voice Privacy Challenge in 2020, along with the release of a framework, the popularity of this research topic is continually increasing. However, the comparison and combination of different anonymization approaches remains challenging due to the complexity of evaluation and the absence of user-friendly research frameworks. We therefore propose an efficient speaker anonymization and evaluation framework based on a modular and easily extendable structure, almost fully in Python. The framework facilitates the orchestration of several anonymization approaches in parallel and allows for interfacing between different techniques. Furthermore, we propose modifications to common evaluation methods which improves the quality of the evaluation and reduces their computation time by 65 to 95%, depending on the metric. Our code is fully open source.

==> bio/bio_texts.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/meyer.jpg}}]{Sarina Meyer} (Student Member, IEEE) is a doctoral student at the Institute for Natural Language Processing at the University of Stuttgart, Germany. She started her Ph.D. in 2021. Her research interests involve privacy and explainability in speech processing, with a particular focus on speaker anonymization.

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/miao.jpg}}]{Xiaoxiao Miao} (Member, IEEE) is an assistant professor at the Singapore Institute of Technology, Singapore. This work was conducted while she was a project researcher at the National Institute of Informatics, Japan. She received the Ph.D. degree from the Institute of Acoustics, Chinese Academy of Sciences/University Chinese Academy of Sciences, in 2021. Her research interests include speaker and language recognition, speech security, and machine learning. She is a co-organizer of the latest VoicePrivacy challenge. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/vu.jpg}}]{Ngoc Thang Vu} (Member, IEEE) is a Full Professor at the Institute for Natural Language Processing at the University of Stuttgart. He received his PhD in computer science (topic: multilingual speech recognition) at the Karlsruhe Institute of Technology (KIT) in 2014. After his PhD, he joined Nuance Communications as a senior research scientist. Later, he became an Acting Professor for computational linguistics at LMU Munich, focusing on natural language processing using deep learning. In 2015, he joined the University of Stuttgart as an Assistant Professor, and in 2018, he was promoted to a full professorship. His research focuses on speech and language processing systems across three dimensions: users (e.g., voice privacy), systems (e.g., controllable and interpretable/explainable systems), and languages (e.g., multilingual systems and adaptation to low-resource languages).

\end{IEEEbiography}
